RobustFed: A Truth Inference Approach for Robust Federated Learning

Federated learning is a prominent framework that enables clients (e.g., mobile devices or organizations) to train a collaboratively global model under a central server's orchestration while keeping local training datasets' privacy. However, the aggregation step in federated learning is vulnerable to adversarial attacks as the central server cannot manage clients' behavior. Therefore, the global model's performance and convergence of the training process will be affected under such attacks.To mitigate this vulnerability issue, we propose a novel robust aggregation algorithm inspired by the truth inference methods in crowdsourcing via incorporating the worker's reliability into aggregation. We evaluate our solution on three real-world datasets with a variety of machine learning models. Experimental results show that our solution ensures robust federated learning and is resilient to various types of attacks, including noisy data attacks, Byzantine attacks, and label flipping attacks.

==> test <==
federated
@inproceedings{fung2020limitations,
  title={The Limitations of Federated Learning in Sybil Settings},
  author={Fung, Clement and Yoon, Chris JM and Beschastnikh, Ivan},
  booktitle={23rd International Symposium on Research in Attacks, Intrusions and Defenses ($\{$RAID$\}$ 2020)},
  pages={301--316},
  year={2020}
}

@article{mothukuri2020survey,
  title={A survey on security and privacy of federated learning},
  author={Mothukuri, Viraaji and Parizi, Reza M and Pouriyeh, Seyedamin and Huang, Yan and Dehghantanha, Ali and Srivastava, Gautam},
  journal={Future Generation Computer Systems},
  year={2020},
  publisher={Elsevier}
}

@incollection{lamport2019byzantine,
  title={The Byzantine generals problem},
  author={Lamport, Leslie and Shostak, Robert and Pease, Marshall},
  booktitle={Concurrency: the Works of Leslie Lamport},
  pages={203--226},
  year={2019}
}



@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial Intelligence and Statistics},
  pages={1273--1282},
  year={2017},
  organization={PMLR}
}

@inproceedings{smith2017federated,
  title={Federated multi-task learning},
  author={Smith, Virginia and Chiang, Chao-Kai and Sanjabi, Maziar and Talwalkar, Ameet S},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4424--4434},
  year={2017}
}

@inproceedings{li2019privacy,
  title={Privacy-preserving federated brain tumour segmentation},
  author={Li, Wenqi and Milletar{\`\i}, Fausto and Xu, Daguang and Rieke, Nicola and Hancox, Jonny and Zhu, Wentao and Baust, Maximilian and Cheng, Yan and Ourselin, S{\'e}bastien and Cardoso, M Jorge and others},
  booktitle={International Workshop on Machine Learning in Medical Imaging},
  pages={133--141},
  year={2019},
  organization={Springer}
}

@article{lim2020federated,
  title={Federated learning in mobile edge networks: A comprehensive survey},
  author={Lim, Wei Yang Bryan and Luong, Nguyen Cong and Hoang, Dinh Thai and Jiao, Yutao and Liang, Ying-Chang and Yang, Qiang and Niyato, Dusit and Miao, Chunyan},
  journal={IEEE Communications Surveys \& Tutorials},
  year={2020},
  publisher={IEEE}
}

@inproceedings{sheller2018multi,
  title={Multi-institutional deep learning modeling without sharing patient data: A feasibility study on brain tumor segmentation},
  author={Sheller, Micah J and Reina, G Anthony and Edwards, Brandon and Martin, Jason and Bakas, Spyridon},
  booktitle={International MICCAI Brainlesion Workshop},
  pages={92--104},
  year={2018},
  organization={Springer}
}

@inproceedings{abadi2016deep,
  title={Deep learning with differential privacy},
  author={Abadi, Martin and Chu, Andy and Goodfellow, Ian and McMahan, H Brendan and Mironov, Ilya and Talwar, Kunal and Zhang, Li},
  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  pages={308--318},
  year={2016}
}


@article{kairouz2019advances,
  title={Advances and open problems in federated learning},
  author={Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Keith and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
  journal={arXiv preprint arXiv:1912.04977},
  year={2019}
} 

%% Attack
@article{biggio2012poisoning,
  title={Poisoning attacks against support vector machines},
  author={Biggio, Battista and Nelson, Blaine and Laskov, Pavel},
  journal={arXiv preprint arXiv:1206.6389},
  year={2012}
}

@inproceedings{damaskinos2019aggregathor,
  title={Aggregathor: Byzantine machine learning via robust gradient aggregation},
  author={Damaskinos, Georgios and El Mhamdi, El Mahdi and Guerraoui, Rachid and Guirguis, Arsany Hany Abdelmessih and Rouault, S{\'e}bastien Louis Alexandre},
  booktitle={The Conference on Systems and Machine Learning (SysML), 2019},
  number={CONF},
  year={2019}
}

@article{gu2019badnets,
  title={Badnets: Evaluating backdooring attacks on deep neural networks},
  author={Gu, Tianyu and Liu, Kang and Dolan-Gavitt, Brendan and Garg, Siddharth},
  journal={IEEE Access},
  volume={7},
  pages={47230--47244},
  year={2019},
  publisher={IEEE}
}

@inproceedings{blanchard2017machine,
  title={Machine learning with adversaries: Byzantine tolerant gradient descent},
  author={Blanchard, Peva and Guerraoui, Rachid and Stainer, Julien and others},
  booktitle={Advances in Neural Information Processing Systems},
  pages={119--129},
  year={2017}
}


@article{fung2018mitigating,
  title={Mitigating sybils in federated learning poisoning},
  author={Fung, Clement and Yoon, Chris JM and Beschastnikh, Ivan},
  journal={arXiv preprint arXiv:1808.04866},
  year={2018}
}

@article{bagdasaryan2018backdoor,
  title={How to backdoor federated learning},
  author={Bagdasaryan, Eugene and Veit, Andreas and Hua, Yiqing and Estrin, Deborah and Shmatikov, Vitaly},
  journal={arXiv preprint arXiv:1807.00459},
  year={2018}
}

@article{fang2019local,
  title={Local Model Poisoning Attacks to Byzantine-Robust Federated Learning},
  author={Fang, Minghong and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  journal={arXiv preprint arXiv:1911.11815},
  year={2019}
}

@inproceedings{bhagoji2019analyzing,
  title={Analyzing Federated Learning through an Adversarial Lens},
  author={Bhagoji, Arjun Nitin and Chakraborty, Supriyo and Mittal, Prateek and Calo, Seraphin},
  booktitle={International Conference on Machine Learning},
  pages={634--643},
  year={2019}
}


@article{lin2019free,
  title={Free-riders in Federated Learning: Attacks and Defenses},
  author={Lin, Jierui and Du, Min and Liu, Jian},
  journal={arXiv preprint arXiv:1911.12560},
  year={2019}
}

@article{munoz2019byzantine,
  title={Byzantine-Robust Federated Machine Learning through Adaptive Model Averaging},
  author={Mu{\~n}oz-Gonz{\'a}lez, Luis and Co, Kenneth T and Lupu, Emil C},
  journal={arXiv preprint arXiv:1909.05125},
  year={2019}
}

@article{zong2018deep,
  title={Deep autoencoding gaussian mixture model for unsupervised anomaly detection},
  author={Zong, Bo and Song, Qi and Min, Martin Renqiang and Cheng, Wei and Lumezanu, Cristian and Cho, Daeki and Chen, Haifeng},
  year={2018}
}


%%Defense
@article{yin2018byzantine,
  title={Byzantine-robust distributed learning: Towards optimal statistical rates},
  author={Yin, Dong and Chen, Yudong and Ramchandran, Kannan and Bartlett, Peter},
  journal={arXiv preprint arXiv:1803.01498},
  year={2018}
}

@article{chen2017distributed,
  title={Distributed statistical machine learning in adversarial settings: Byzantine gradient descent},
  author={Chen, Yudong and Su, Lili and Xu, Jiaming},
  journal={Proceedings of the ACM on Measurement and Analysis of Computing Systems},
  volume={1},
  number={2},
  pages={1--25},
  year={2017},
  publisher={ACM New York, NY, USA}
}

%truth_inference
@inproceedings{li2014resolving,
  title={Resolving conflicts in heterogeneous data by truth discovery and source reliability estimation},
  author={Li, Qi and Li, Yaliang and Gao, Jing and Zhao, Bo and Fan, Wei and Han, Jiawei},
  booktitle={Proceedings of the 2014 ACM SIGMOD international conference on Management of data},
  pages={1187--1198},
  year={2014},
  organization={ACM}
}



@article{bagdasaryan2018backdoor,
  title={How to backdoor federated learning},
  author={Bagdasaryan, Eugene and Veit, Andreas and Hua, Yiqing and Estrin, Deborah and Shmatikov, Vitaly},
  journal={arXiv preprint arXiv:1807.00459},
  year={2018}
}

@article{lin2019free,
  title={Free-riders in Federated Learning: Attacks and Defenses},
  author={Lin, Jierui and Du, Min and Liu, Jian},
  journal={arXiv preprint arXiv:1911.12560},
  year={2019}
}

@article{zong2018deep,
  title={Deep autoencoding gaussian mixture model for unsupervised anomaly detection},
  author={Zong, Bo and Song, Qi and Min, Martin Renqiang and Cheng, Wei and Lumezanu, Cristian and Cho, Daeki and Chen, Haifeng},
  year={2018}
}

@article{lim2019federated,
  title={Federated Learning in Mobile Edge Networks: A Comprehensive Survey},
  author={Lim, Wei Yang Bryan and Luong, Nguyen Cong and Hoang, Dinh Thai and Jiao, Yutao and Liang, Ying-Chang and Yang, Qiang and Niyato, Dusit and Miao, Chunyan},
  journal={arXiv preprint arXiv:1909.11875},
  year={2019}
}


@article{fang2019local,
  title={Local Model Poisoning Attacks to Byzantine-Robust Federated Learning},
  author={Fang, Minghong and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  journal={arXiv preprint arXiv:1911.11815},
  year={2019}
}
%truth inference

@inproceedings{tahmasebian2020crowdsourcing,
  title={Crowdsourcing under data poisoning attacks: A comparative study},
  author={Tahmasebian, Farnaz and Xiong, Li and Sotoodeh, Mani and Sunderam, Vaidy},
  booktitle={IFIP Annual Conference on Data and Applications Security and Privacy},
  pages={310--332},
  year={2020},
  organization={Springer}
}

@inproceedings{gaunt2016training,
  title={Training deep neural nets to aggregate crowdsourced responses},
  author={Gaunt, Alex and Borsa, Diana and Bachrach, Yoram},
  booktitle={Proceedings of the Thirty-Second Conference on Uncertainty in Artificial Intelligence. AUAI Press},
  pages={242251},
  year={2016}
}

@inproceedings{liaggregating,
  title={Aggregating crowd wisdoms with label-aware autoencoders},
  author={Yin, Li'ang and Han, Jianhua and Zhang, Weinan and Yu, Yong},
  booktitle={Proceedings of the 26th International Joint Conference on Artificial Intelligence},
  pages={1325--1331},
  year={2017},
  organization={AAAI Press}
}



@inproceedings{zhou2016crowdsourcing,
  title={Crowdsourcing via Tensor Augmentation and Completion.},
  author={Zhou, Yao and He, Jingrui},
  booktitle={IJCAI},
  pages={2435--2441},
  year={2016}
}

@inproceedings{jagabathula2014reputation,
  title={Reputation-based worker filtering in crowdsourcing},
  author={Jagabathula, Srikanth and Subramanian, Lakshminarayanan and Venkataraman, Ashwin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2492--2500},
  year={2014}
}


@article{zheng2017truth,
  title={Truth inference in crowdsourcing: is the problem solved?},
  author={Zheng, Yudian and Li, Guoliang and Li, Yuanbing and Shan, Caihua and Cheng, Reynold},
  journal={Proceedings of the VLDB Endowment},
  volume={10},
  number={5},
  pages={541--552},
  year={2017},
  publisher={VLDB Endowment}
}

@article{dawid1979maximum,
  title={Maximum likelihood estimation of observer error-rates using the EM algorithm},
  author={Dawid, Alexander Philip and Skene, Allan M},
  journal={Applied statistics},
  pages={20--28},
  year={1979},
  publisher={JSTOR}
}

@inproceedings{karger2011iterative,
  title={Iterative learning for reliable crowdsourcing systems},
  author={Karger, David R and Oh, Sewoong and Shah, Devavrat},
  booktitle={Advances in neural information processing systems},
  pages={1953--1961},
  year={2011}
}



@inproceedings{demartini2012zencrowd,
  title={ZenCrowd: leveraging probabilistic reasoning and crowdsourcing techniques for large-scale entity linking},
  author={Demartini, Gianluca and Difallah, Djellel Eddine and Cudr{\'e}-Mauroux, Philippe},
  booktitle={Proceedings of the 21st international conference on World Wide Web},
  pages={469--478},
  year={2012},
  organization={ACM}
}

@inproceedings{whitehill2009whose,
  title={Whose vote should count more: Optimal integration of labels from labelers of unknown expertise},
  author={Whitehill, Jacob and Wu, Ting-fan and Bergsma, Jacob and Movellan, Javier R and Ruvolo, Paul L},
  booktitle={Advances in neural information processing systems},
  pages={2035--2043},
  year={2009}
}

@inproceedings{venanzi2014community,
  title={Community-based bayesian aggregation models for crowdsourcing},
  author={Venanzi, Matteo and Guiver, John and Kazai, Gabriella and Kohli, Pushmeet and Shokouhi, Milad},
  booktitle={Proceedings of the 23rd international conference on World Wide Web},
  pages={155--164},
  year={2014},
  organization={ACM}
}

@inproceedings{kim2012bayesian,
  title={Bayesian classifier combination},
  author={Kim, Hyun-Chul and Ghahramani, Zoubin},
  booktitle={Artificial Intelligence and Statistics},
  pages={619--627},
  year={2012}
}

@inproceedings{zhou2012learning,
  title={Learning from the wisdom of crowds by minimax entropy},
  author={Zhou, Dengyong and Basu, Sumit and Mao, Yi and Platt, John C},
  booktitle={Advances in neural information processing systems},
  pages={2195--2203},
  year={2012}
}


@inproceedings{zhou2017multic2,
  title={MultiC2: an optimization framework for learning from task and worker dual heterogeneity},
  author={Zhou, Yao and Ying, Lei and He, Jingrui},
  booktitle={Proceedings of the 2017 SIAM International Conference on Data Mining},
  pages={579--587},
  year={2017},
  organization={SIAM}
}

@article{li2014confidence,
  title={A confidence-aware approach for truth discovery on long-tail data},
  author={Li, Qi and Li, Yaliang and Gao, Jing and Su, Lu and Zhao, Bo and Demirbas, Murat and Fan, Wei and Han, Jiawei},
  journal={Proceedings of the VLDB Endowment},
  volume={8},
  number={4},
  pages={425--436},
  year={2014},
  publisher={VLDB Endowment}
}

@article{zhao2012bayesian,
  title={A bayesian approach to discovering truth from conflicting sources for data integration},
  author={Zhao, Bo and Rubinstein, Benjamin IP and Gemmell, Jim and Han, Jiawei},
  journal={Proceedings of the VLDB Endowment},
  volume={5},
  number={6},
  pages={550--561},
  year={2012},
  publisher={VLDB Endowment}
}


@article{jwang2012crowd,
  title={Crowdsourcing entity resolution},
  author={ J. Wang, T. Kraska, M. J. Franklin, and J. Feng. Crowderd},
  journal={PVLDB},
  volume={5},
  number={11},
  pages={1483–1494},
  year={2012},
  publisher={VLDB Endowment}
}

@article{raykar2010learning,
  title={Learning from crowds},
  author={Raykar, Vikas C and Yu, Shipeng and Zhao, Linda H and Valadez, Gerardo Hermosillo and Florin, Charles and Bogoni, Luca and Moy, Linda},
  journal={Journal of Machine Learning Research},
  volume={11},
  number={Apr},
  pages={1297--1322},
  year={2010}
}

@inproceedings{kittur2008crowdsourcing,
  title={Crowdsourcing user studies with Mechanical Turk},
  author={Kittur, Aniket and Chi, Ed H and Suh, Bongwon},
  booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
  pages={453--456},
  year={2008},
  organization={ACM}
}



%Byzantine-robust Aggregation Rules



@inproceedings{guerraoui2018hidden,
  title={The hidden vulnerability of distributed learning in byzantium},
  author={Guerraoui, Rachid and Rouault, S{\'e}bastien and others},
  booktitle={International Conference on Machine Learning},
  pages={3521--3530},
  year={2018},
  organization={PMLR}
}

@inproceedings{alistarh2018byzantine,
  title={Byzantine stochastic gradient descent},
  author={Alistarh, Dan and Allen-Zhu, Zeyuan and Li, Jerry},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4613--4623},
  year={2018}
}

@inproceedings{li2019rsa,
  title={RSA: Byzantine-robust stochastic aggregation methods for distributed learning from heterogeneous datasets},
  author={Li, Liping and Xu, Wei and Chen, Tianyi and Giannakis, Georgios B and Ling, Qing},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={1544--1551},
  year={2019}
}

@inproceedings{xie2019dba,
  title={Dba: Distributed backdoor attacks against federated learning},
  author={Xie, Chulin and Huang, Keli and Chen, Pin-Yu and Li, Bo},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{wang2019neural,
  title={Neural cleanse: Identifying and mitigating backdoor attacks in neural networks},
  author={Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={707--723},
  year={2019},
  organization={IEEE}
}
@article{sattler2019robust,
  title={Robust and communication-efficient federated learning from non-iid data},
  author={Sattler, Felix and Wiedemann, Simon and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  journal={IEEE transactions on neural networks and learning systems},
  volume={31},
  number={9},
  pages={3400--3413},
  year={2019},
  publisher={IEEE}
}
